GeoGaussian: Geometry-aware Gaussian Splatting for Scene Rendering

During the Gaussian Splatting optimization process, the scene's geometry can gradually deteriorate if its structure is not deliberately preserved, especially in non-textured regions such as walls, ceilings, and furniture surfaces. This degradation significantly affects the rendering quality of novel views that deviate significantly from the viewpoints in the training data. To mitigate this issue, we propose a novel approach called GeoGaussian. Based on the smoothly connected areas observed from point clouds, this method introduces a novel pipeline to initialize thin Gaussians aligned with the surfaces, where the characteristic can be transferred to new generations through a carefully designed densification strategy. Finally, the pipeline ensures that the scene's geometry and texture are maintained through constrained optimization processes with explicit geometry constraints. Benefiting from the proposed architecture, the generative ability of 3D Gaussians is enhanced, especially in structured regions. Our proposed pipeline achieves state-of-the-art performance in novel view synthesis and geometric reconstruction, as evaluated qualitatively and quantitatively on public datasets.

==> tables/ablation.tex <==
\newcommand{\tablestyle}[2]{\setlength{\tabcolsep}{#1}\renewcommand{\arraystretch}{#2}\centering\footnotesize}
\begin{table}[!ht]
    \centering
    \begin{tabular}{c|cc|c|c|cc|cc}
        No. & $F_{conv}$ & $F_{dino}$ & $\sigma$ & SAP & $NIoU_{25}$ & $NIoU_{50}$ & $10^\circ 0.2d$ & $10^\circ 0.5d$ \\ \hline
        A & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ 
        B & \checkmark & ~ & ~ & \checkmark & ~ & ~ & ~ & ~ \\ 
        C &  & \checkmark & ~ & \checkmark & ~ & ~ & ~ & ~ \\ 
        D & \checkmark & \checkmark & ~ & \checkmark & ~ & ~ & ~ & ~ \\ 
        E & \checkmark & \checkmark & \checkmark & ~ & ~ & ~ & ~ & ~ \\
        F & \checkmark &\checkmark & \checkmark & \checkmark & ~ & ~ & ~ & ~ \\
        % G & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ 
    \end{tabular}
    \label{tab: ablation}
    \caption{Ablation studies on NOCS-REAL275. $\sigma$ denotes whether uncertainty maps are used to guide PnP module. SAP denotes whether scale-agnostic pose representation are used.}
\end{table}

==> tables/abs_result.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c c c|c c c c c}
        Method & $IoU_{25}$ & $IoU_{50}$ & $IoU_{75}$ & $10^\circ 10cm$ & $10cm$ \\ \hline
        MSOS \cite{lee2021msos} & 33.2 & 13.6 & 1.0 & 11.8 & 43.4   \\ 
        OLD-Net \cite{fan2022oldnet} & 26.4 & 7.7 & 0.4 & 8.6 & 31.4  \\
        DMSR \cite{wei2023dmsr} & 37.4 & 16.3 & \textbf{3.2} & 25.2 & 40.0   \\ 
         \hline
        Ours  & 40.0 & \textbf{18.5} & 2.5 & \textbf{31.0} & \textbf{46.2}  \\ 
        Ours (M) & \textbf{41.0} & 18.2 & \textbf{3.2} & 27.1 & 43.8 \\ 
    \end{tabular}
    \caption{Comparison with state-of-the-art methods on NOCS-REAL275 using evaluation metrics with absolute object scale.}
    \label{tab:abs}
\end{table}

==> tables/camera_result.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c c c|c c c c c}
        Method & $NIoU_{25}$ & $NIoU_{50}$ & $NIoU_{75}$ & $10^\circ 0.2d$ & $10^\circ 0.5d$ & $10^\circ$ & $0.2d$ & $0.5d$ \\ \hline
        MSOS \cite{lee2021msos} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ 
        OLD-Net \cite{fan2022oldnet} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\
        DMSR \cite{wei2023dmsr} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ 
         \hline
        Ours & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ 
        Ours (M) & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ 
    \end{tabular}
    \caption{Comparison with state-of-the-art methods on NOCS-CAMERA25  using scale-agnostic evaluation metrics.}
    \label{tab:camera}
\end{table}

==> tables/norm_result.tex <==
\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{1mm}
    \begin{tabular}{c|c c c|c c c c c}
        Method & $NIoU_{25}$ & $NIoU_{50}$ & $NIoU_{75}$ & $10^\circ 0.2d$ & $10^\circ 0.5d$ & $0.2d$ & $0.5d$ & $10^\circ$ \\ \hline
        MSOS \cite{lee2021msos} & 36.9 & 9.7 & 0.7 & 3.3 & 15.3 & 10.6 & 50.8 & 17.0 \\ 
        OLD-Net \cite{fan2022oldnet} & 31.5 & 6.2 & 0.1 & 2.8 & 12.2 & 9.0 & 44.0 & 14.8 \\
        DMSR \cite{wei2023dmsr} & 57.2 & 38.4 & 9.7 & 26.0 & 44.9 & 35.8 & 67.2 & 36.9 \\ 
         \hline
        Ours  & 65.5 & 44.9 & 13.2 & 36.4 & 54.0 & 43.7 & 74.1 & 58.1 \\ 
        Ours (M) & \textbf{67.4} & \textbf{48.9} & \textbf{21.1} & \textbf{39.3} & \textbf{54.9} & \textbf{49.0} & \textbf{76.5} & \textbf{58.6} \\ 
    \end{tabular}
    \caption{Comparison with state-of-the-art methods on NOCS-REAL275 using scale-agnostic evaluation metrics.}
    \label{tab:norm}
\end{table}
